Equity-Transformer: Solving NP-hard Min-Max Routing Problems as Sequential Generation with Equity Context

Min-max routing problems aim to minimize the maximum tour length among multiple agents by having agents conduct tasks in a cooperative manner. These problems include impactful real-world applications but are known as NP-hard. Existing methods are facing challenges, particularly in large-scale problems that require the coordination of numerous agents to cover thousands of cities. This paper proposes Equity-Transformer to solve large-scale min-max routing problems. First, we employ sequential planning approach to address min-max routing problems, allowing us to harness the powerful sequence generators (e.g., Transformer). Second, we propose key inductive biases that ensure equitable workload distribution among agents. The effectiveness of Equity-Transformer is demonstrated through its superior performance in two representative min-max routing tasks: the min-max multi-agent traveling salesman problem (min-max mTSP) and the min-max multi-agent pick-up and delivery problem (min-max mPDP). Notably, our method achieves significant reductions of runtime, approximately 335 times, and cost values of about 53\% compared to a competitive heuristic (LKH3) in the case of 100 vehicles with 1,000 cities of mTSP. We provide reproducible source code: \url{https://github.com/kaist-silab/equity-transformer}.

==> tables/table3.tex <==
\begin{table*}[h]
\begin{center}
% \caption{
% {Performance evaluation results on mTSP synthetic dataset. Every performance is average performance among 100 instances. The bold symbol indicates best performance and the underline indicates second and third place. Running times (in minutes) are provided in brackets.  
% }
% }
\vspace{0.01in}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{
c 
c
c  
c 
c 
c 
c 
c 
c
}
\toprule
&
& \multicolumn{2}{c}{Classic-based}
& \multicolumn{4}{c}{Learning-based}
%& \multicolumn{1}{c}{Ours}
\\
\cmidrule(lr{0.2em}){3-4}
\cmidrule(lr{0.2em}){5-8} 
% \cmidrule(lr{0.2em}){9-9}
\multicolumn{1}{c}{TSPLib}
& \multicolumn{1}{c}{$M$} 
& \multicolumn{1}{c}{LKH3}
% & \multicolumn{1}{c}{LKH3 (10)}
& \multicolumn{1}{c}{OR-tools}
% & \multicolumn{1}{c}{OR-tools (10)}
& \multicolumn{1}{c}{SN \cite{park2021schedulenet}}
& \multicolumn{1}{c}{NCE \cite{nce}}
% & \multicolumn{1}{c}{MF (N.C.)}
& \multicolumn{1}{c}{ET (ours)}
& \multicolumn{1}{c}{ET$^\dagger$(ours)}
\\
\midrule

\multirow{3.5}{*}{\shortstack[l]{Eil51}}
&5
% &2.52 \small{(102)}
% &- \small{(-)}
&4.55 \small{(100)}
&- \small{(-)}
&2.35 \small{(16.67)}
&120.67 \small{(1.85)}
% &2.15 \small{(0.03)}
&\textbf{120.0} \small{(1.65)}

\\
\addlinespace
&7
% &2.39 \small{(102)}
% &- \small{(-)}
&4.56 \small{(100)}
&- \small{(-)}
&2.13 \small{(17.53)}
&112.1 \small{(1.27)}
% &1.99 \small{(0.03)}
&\textbf{112.1} \small{(1.20)}

\\
\addlinespace
&10
% &2.29 \small{(102)}
% &- \small{(-)}
&4.57 \small{(100)}
&- \small{(-)}
&2.07 \small{(19.00)}
&112.1 \small{(1.98)}
% &1.98 \small{(0.03)}
&\textbf{112.1} \small{(1.42)}

\\
\midrule
\multirow{3.5}{*}{\shortstack[l]{Berlin52}}
&5
% &3.31 \small{(102)}
% &2.70 \small{(1008)}
&- \small{(-)}
&8.45 \small{(1000)}
&2.16 \small{(284.51)}
&2.07 \small{(8.66)}
% &2.40 \small{(0.05)}
&\textbf{2.02} \small{(0.05)}

\\
\addlinespace
&7
% &3.10 \small{(102)}
% &2.55 \small{(1008)}
&- \small{(-)}
&8.18 \small{(1000)}
&2.12 \small{(459.50)}
&2.01 \small{(8.97)}
% &2.22 \small{(0.05)}
&\textbf{2.01} \small{(0.05)}

\\
\addlinespace
&10 
% &2.93 \small{(1002)}
% &2.48 \small{(1008)}
&- \small{(-)}
&8.14 \small{(1000)}
&2.09 \small{(362.20)}
&2.01 \small{(8.41)}
% &2.14 \small{(0.05)}
&\textbf{2.01} \small{(0.05)}

\\
\midrule
\multirow{3.5}{*}{\shortstack[l]{Eil76}}
&5
% &4.45 \small{(102)}
% &3.77 \small{(1005)}
&- \small{(-)}
&14.57 \small{(1000)}
&2.26 \small{(3490)}
&2.13 \small{(25.08)}
% &3.03 \small{(0.13)}
&\textbf{2.06} \small{(0.13)}

\\
\addlinespace
&7
% &3.71 \small{(102)}
% &3.26 \small{(1006)}
&- \small{(-)}
&14.02 \small{(1000)}
&2.17 \small{(2796)}
&2.07 \small{(25.09

)}
% &2.39 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}

\\
\addlinespace
&10
% &3.23 \small{(103)}
% &2.92 \small{(1007)}
&- \small{(-)}
&13.98 \small{(1000)}
&0.00 \small{(0.00)}
&2.05 \small{(25.02)}
% &2.30 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}
\\
\midrule
\multirow{3.5}{*}{\shortstack[l]{Rat99}}
&5
% &- \small{(-)}
% &- \small{(-)}
&- \small{(-)}
&- \small{(-)}
&\textit{OB}
&2.85 \small{(73.26)}
% &2.40 \small{(0.05)}
&\textbf{2.10} \small{(0.78)}

\\
\addlinespace
&7
% &- \small{(-)}
% &- \small{(-)}
&- \small{(-)}
&- \small{(-)}
&\textit{OB}
&2.83 \small{(74.61)}
% &2.22 \small{(0.05)}
&\textbf{2.08} \small{(0.81)}

\\
\addlinespace
&10
% &- \small{(-)}
% &- \small{(-)}
&- \small{(-)}
&- \small{(-)}
&\textit{OB}
&2.08 \small{(50.50)}
% &2.14 \small{(0.05)}
&\textbf{2.08} \small{(0.83)}

\\
\midrule

\multirow{3.5}{*}{\shortstack[l]{kroD100}}
&5
% &4.45 \small{(102)}
% &3.77 \small{(1005)}
&- \small{(-)}
&14.57 \small{(1000)}
&2.26 \small{(3490)}
&2.13 \small{(25.08)}
% &3.03 \small{(0.13)}
&\textbf{2.06} \small{(0.13)}

\\
\addlinespace
&10
% &3.71 \small{(102)}
% &3.26 \small{(1006)}
&- \small{(-)}
&14.02 \small{(1000)}
&2.17 \small{(2796)}
&2.07 \small{(25.09

)}
% &2.39 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}

\\
\addlinespace
&15
% &3.23 \small{(103)}
% &2.92 \small{(1007)}
&- \small{(-)}
&13.98 \small{(1000)}
&0.00 \small{(0.00)}
&2.05 \small{(25.02)}
% &2.30 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}
\\
\midrule

\multirow{3.5}{*}{\shortstack[l]{ch150}}
&5
% &4.45 \small{(102)}
% &3.77 \small{(1005)}
&- \small{(-)}
&14.57 \small{(1000)}
&2.26 \small{(3490)}
&2.13 \small{(25.08)}
% &3.03 \small{(0.13)}
&\textbf{2.06} \small{(0.13)}

\\
\addlinespace
&10
% &3.71 \small{(102)}
% &3.26 \small{(1006)}
&- \small{(-)}
&14.02 \small{(1000)}
&2.17 \small{(2796)}
&2.07 \small{(25.09

)}
% &2.39 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}

\\
\addlinespace
&15
% &3.23 \small{(103)}
% &2.92 \small{(1007)}
&- \small{(-)}
&13.98 \small{(1000)}
&0.00 \small{(0.00)}
&2.05 \small{(25.02)}
% &2.30 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}
\\
\midrule

\multirow{3.5}{*}{\shortstack[l]{kroA200}}
&10
% &4.45 \small{(102)}
% &3.77 \small{(1005)}
&- \small{(-)}
&14.57 \small{(1000)}
&2.26 \small{(3490)}
&2.13 \small{(25.08)}
% &3.03 \small{(0.13)}
&\textbf{2.06} \small{(0.13)}

\\
\addlinespace
&15
% &3.71 \small{(102)}
% &3.26 \small{(1006)}
&- \small{(-)}
&14.02 \small{(1000)}
&2.17 \small{(2796)}
&2.07 \small{(25.09

)}
% &2.39 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}

\\
\addlinespace
&20
% &3.23 \small{(103)}
% &2.92 \small{(1007)}
&- \small{(-)}
&13.98 \small{(1000)}
&0.00 \small{(0.00)}
&2.05 \small{(25.02)}
% &2.30 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}
\\
\midrule

\multirow{3.5}{*}{\shortstack[l]{lin318}}
&10
% &4.45 \small{(102)}
% &3.77 \small{(1005)}
&- \small{(-)}
&14.57 \small{(1000)}
&2.26 \small{(3490)}
&2.13 \small{(25.08)}
% &3.03 \small{(0.13)}
&\textbf{2.06} \small{(0.13)}

\\
\addlinespace
&15
% &3.71 \small{(102)}
% &3.26 \small{(1006)}
&- \small{(-)}
&14.02 \small{(1000)}
&2.17 \small{(2796)}
&2.07 \small{(25.09

)}
% &2.39 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}

\\
\addlinespace
&20
% &3.23 \small{(103)}
% &2.92 \small{(1007)}
&- \small{(-)}
&13.98 \small{(1000)}
&0.00 \small{(0.00)}
&2.05 \small{(25.02)}
% &2.30 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}
\\
\midrule

\multirow{3.5}{*}{\shortstack[l]{att532}}
&30
% &4.45 \small{(102)}
% &3.77 \small{(1005)}
&- \small{(-)}
&14.57 \small{(1000)}
&2.26 \small{(3490)}
&2.13 \small{(25.08)}
% &3.03 \small{(0.13)}
&\textbf{2.06} \small{(0.13)}

\\
\addlinespace
&40
% &3.71 \small{(102)}
% &3.26 \small{(1006)}
&- \small{(-)}
&14.02 \small{(1000)}
&2.17 \small{(2796)}
&2.07 \small{(25.09

)}
% &2.39 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}

\\
\addlinespace
&50
% &3.23 \small{(103)}
% &2.92 \small{(1007)}
&- \small{(-)}
&13.98 \small{(1000)}
&0.00 \small{(0.00)}
&2.05 \small{(25.02)}
% &2.30 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}
\\
\midrule

\multirow{3.5}{*}{\shortstack[l]{rat783}}
&30
% &4.45 \small{(102)}
% &3.77 \small{(1005)}
&- \small{(-)}
&14.57 \small{(1000)}
&2.26 \small{(3490)}
&2.13 \small{(25.08)}
% &3.03 \small{(0.13)}
&\textbf{2.06} \small{(0.13)}

\\
\addlinespace
&40
% &3.71 \small{(102)}
% &3.26 \small{(1006)}
&- \small{(-)}
&14.02 \small{(1000)}
&2.17 \small{(2796)}
&2.07 \small{(25.09

)}
% &2.39 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}

\\
\addlinespace
&50
% &3.23 \small{(103)}
% &2.92 \small{(1007)}
&- \small{(-)}
&13.98 \small{(1000)}
&0.00 \small{(0.00)}
&2.05 \small{(25.02)}
% &2.30 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}
\\
\midrule

\multirow{3.5}{*}{\shortstack[l]{pcb1173}}
&50
% &4.45 \small{(102)}
% &3.77 \small{(1005)}
&- \small{(-)}
&14.57 \small{(1000)}
&2.26 \small{(3490)}
&2.13 \small{(25.08)}
% &3.03 \small{(0.13)}
&\textbf{2.06} \small{(0.13)}

\\
\addlinespace
&75
% &3.71 \small{(102)}
% &3.26 \small{(1006)}
&- \small{(-)}
&14.02 \small{(1000)}
&2.17 \small{(2796)}
&2.07 \small{(25.09

)}
% &2.39 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}

\\
\addlinespace
&100
% &3.23 \small{(103)}
% &2.92 \small{(1007)}
&- \small{(-)}
&13.98 \small{(1000)}
&0.00 \small{(0.00)}
&2.05 \small{(25.02)}
% &2.30 \small{(0.14)}
&\textbf{2.05} \small{(0.14)}
\\
\midrule

% \multirow{3.5}{*}{\shortstack[l]{Eil76}}
% &5
% % &4.45 \small{(102)}
% % &3.77 \small{(1005)}
% &- \small{(-)}
% &14.57 \small{(1000)}
% &2.26 \small{(3490)}
% &2.13 \small{(25.08)}
% % &3.03 \small{(0.13)}
% &\textbf{2.06} \small{(0.13)}

% \\
% \addlinespace
% &7
% % &3.71 \small{(102)}
% % &3.26 \small{(1006)}
% &- \small{(-)}
% &14.02 \small{(1000)}
% &2.17 \small{(2796)}
% &2.07 \small{(25.09

% )}
% % &2.39 \small{(0.14)}
% &\textbf{2.05} \small{(0.14)}

% \\
% \addlinespace
% &10
% % &3.23 \small{(103)}
% % &2.92 \small{(1007)}
% &- \small{(-)}
% &13.98 \small{(1000)}
% &0.00 \small{(0.00)}
% &2.05 \small{(25.02)}
% % &2.30 \small{(0.14)}
% &\textbf{2.05} \small{(0.14)}
% \\
% \midrule

% \multirow{3.5}{*}{\shortstack[l]{Eil76}}
% &5
% % &4.45 \small{(102)}
% % &3.77 \small{(1005)}
% &- \small{(-)}
% &14.57 \small{(1000)}
% &2.26 \small{(3490)}
% &2.13 \small{(25.08)}
% % &3.03 \small{(0.13)}
% &\textbf{2.06} \small{(0.13)}

% \\
% \addlinespace
% &7
% % &3.71 \small{(102)}
% % &3.26 \small{(1006)}
% &- \small{(-)}
% &14.02 \small{(1000)}
% &2.17 \small{(2796)}
% &2.07 \small{(25.09

% )}
% % &2.39 \small{(0.14)}
% &\textbf{2.05} \small{(0.14)}

% \\
% \addlinespace
% &10
% % &3.23 \small{(103)}
% % &2.92 \small{(1007)}
% &- \small{(-)}
% &13.98 \small{(1000)}
% &0.00 \small{(0.00)}
% &2.05 \small{(25.02)}
% % &2.30 \small{(0.14)}
% &\textbf{2.05} \small{(0.14)}
% \\
% \midrule

% \multirow{3.5}{*}{\shortstack[l]{Eil76}}
% &5
% % &4.45 \small{(102)}
% % &3.77 \small{(1005)}
% &- \small{(-)}
% &14.57 \small{(1000)}
% &2.26 \small{(3490)}
% &2.13 \small{(25.08)}
% % &3.03 \small{(0.13)}
% &\textbf{2.06} \small{(0.13)}

% \\
% \addlinespace
% &7
% % &3.71 \small{(102)}
% % &3.26 \small{(1006)}
% &- \small{(-)}
% &14.02 \small{(1000)}
% &2.17 \small{(2796)}
% &2.07 \small{(25.09

% )}
% % &2.39 \small{(0.14)}
% &\textbf{2.05} \small{(0.14)}

% \\
% \addlinespace
% &10
% % &3.23 \small{(103)}
% % &2.92 \small{(1007)}
% &- \small{(-)}
% &13.98 \small{(1000)}
% &0.00 \small{(0.00)}
% &2.05 \small{(25.02)}
% % &2.30 \small{(0.14)}
% &\textbf{2.05} \small{(0.14)}
% \\
% \midrule

% \multirow{3.5}{*}{\shortstack[l]{Eil76}}
% &5
% % &4.45 \small{(102)}
% % &3.77 \small{(1005)}
% &- \small{(-)}
% &14.57 \small{(1000)}
% &2.26 \small{(3490)}
% &2.13 \small{(25.08)}
% % &3.03 \small{(0.13)}
% &\textbf{2.06} \small{(0.13)}

% \\
% \addlinespace
% &7
% % &3.71 \small{(102)}
% % &3.26 \small{(1006)}
% &- \small{(-)}
% &14.02 \small{(1000)}
% &2.17 \small{(2796)}
% &2.07 \small{(25.09

% )}
% % &2.39 \small{(0.14)}
% &\textbf{2.05} \small{(0.14)}

% \\
% \addlinespace
% &10
% % &3.23 \small{(103)}
% % &2.92 \small{(1007)}
% &- \small{(-)}
% &13.98 \small{(1000)}
% &0.00 \small{(0.00)}
% &2.05 \small{(25.02)}
% % &2.30 \small{(0.14)}
% &\textbf{2.05} \small{(0.14)}
% \\
% \midrule




\multirow{3.5}{*}{\shortstack[l]{d1655}}
&50
% &- \small{(-)}
% &- \small{(-)}
&- \small{(-)}
&- \small{(-)}
&\textit{OB}
&2.97 \small{(483)}
% &3.03 \small{(0.13)}
&\textbf{2.40} \small{(8.09)}

\\
\addlinespace
&75
% &- \small{(-)}
% &- \small{(-)}
&- \small{(-)}
&- \small{(-)}
&\textit{OB}
&2.92 \small{(340)}
% &2.39 \small{(0.14)}
&\textbf{2.21} \small{(8.35)}

\\
\addlinespace
&100
% &- \small{(-)}
% &- \small{(-)}
&- \small{(-)}
&- \small{(-)}
&\textit{OB}
&2.89 \small{(330)}
% &2.30 \small{(0.14)}
&\textbf{2.19} \small{(8.60)}

\\
\bottomrule
\end{tabular}%
}
\vspace{-15pt}
\end{center}
\label{tab:mtsplib}
\end{table*}
